Local Pan-Privacy for Federated Analytics

Pan-privacy was proposed by Dwork et al. as an approach to designing a private analytics system that retains its privacy properties in the face of intrusions that expose the system's internal state. Motivated by federated telemetry applications, we study local pan-privacy, where privacy should be retained under repeated unannounced intrusions on the local state. We consider the problem of monitoring the count of an event in a federated system, where event occurrences on a local device should be hidden even from an intruder on that device. We show that under reasonable constraints, the goal of providing information-theoretic differential privacy under intrusion is incompatible with collecting telemetry information. We then show that this problem can be solved in a scalable way using standard cryptographic primitives.

==> Sections/pseudocode.tex <==
\section{Deferred Pseudocode for algorithms}
\label{app:pseudocode}
\begin{figure}[!h]
\begin{algorithm}[H]
\caption{Counter, Client Algorithm}\label{alg:histograms}
    \begin{algorithmic}[1]
    \Require $k, T, \enc, \rerandomize, \x = x_1,x_2,\ldots,x_T$.
    \State \underline{\textbf{Initialization}}
    \State $c_0=\enc(1)$; $d_0=\enc(1)$
    \For{$i=1:k$}
        \State $c_i=\enc(0)$; $d_i = \enc(0)$
    \EndFor
    \vspace{0.1in}

    \State \underline{\textbf{State Update}}
    \For{$t=1:T$}
       \If{$x_t = 0$}
        \For{$i=0:k$}
            \State $c_i=\rerandomize(c_i)$, $d_i=\rerandomize(d_i)$.
        \EndFor
       \Else% \If{$t\in\texttt{Updates}$}
            \State $c_0=\rerandomize^{t}(\enc(0))$; $d_0=\rerandomize^t(\enc(1))$
            \For{$i=1:k$}
                \State $c_i=\rerandomize(c_{i-1})$; $d_i=\rerandomize(d_{i-1})$
            \EndFor
        \EndIf
    \EndFor
    \vspace{0.1in}

    \State \underline{\textbf{Send to Server}}
    \For{$i=0:k-1$}
        \State $v_i=\rerandomize(c_i)$
    \EndFor
    \State $v_k = \rerandomize(d_k)$
    \For{$i=0:k$}
        \State $r={\rm Ber}(2/(e^{\epsilon_0}+1)$
        \If{$r=0$}
            \State $r'={\rm Ber}(1/2)$
            \If{$r'=1$}
                \State $v_i=\rerandomize^{T+1}(\enc(0))$
            \Else
                \State $v_i=\rerandomize^{T+1}(\enc(1))$
            \EndIf
        \EndIf
    \EndFor

    \State \textbf{Return} $(v_0, \ldots, v_k)$
    \end{algorithmic}
\end{algorithm}
\end{figure}

 \algrenewcommand\algorithmicindent{1.0em}%
 \begin{figure}[!h]
\begin{algorithm}[H]
\caption{\countnonzero, Client Algorithm, Two-server model}\label{localpanprivcounting2s}
    \begin{algorithmic}[1]
    \Require $T, \enci{1}, \rerandomizei{1}, \enci{2}, \rerandomizei{2}, \x=x_1,\ldots,x_T$
    \State \underline{\textbf{Initialization}}
    \State $(\si{1},\si{2})=\secretshare(0)$
    \State $(\pi^{(1)}, \pi^{(2)}) = \validityproof(\si{1},\si{2})$
    \State $(\ci{1}, \ci{2}) = (\enci{1}(\si{1}), \enci{2}(\si{2}))$
    \State $(\pri{1},\pri{2}) = (\enci{1}(\pi^{(1)}),  \enci{2}(\pi^{(2)}))$
    
%    \State $(c_{\rm helper}, c_{\rm leader})=(\enc_{\rm helper}(s_{\rm helper}), \enc_{\rm leader}(s_{\rm leader}))$
    \vspace{0.1in}

    \State \underline{\textbf{State Update}}
    \For{$t=1:T$}
        \If{$x_t = 1$}
            \State $(\si{1},\si{2})=\secretshare(1)$ \label{step:newshare}
            %\State $(s_{\rm helper}, s_{\rm leader})=\secretshare(1)$
  \State $(\pi^{(1)}, \pi^{(2)}) = \validityproof(\si{1},\si{2})$
    \State $(\ci{1}, \ci{2}) = (\rerandomizei{1}^t(\enci{1}(\si{1})), \rerandomizei{2}^t(\enci{2}(\si{2})))$
    \State $(\pri{1},\pri{2}) = (\rerandomizei{1}^t(\enci{1}(\pi^{(1)})),  \rerandomizei{2}^t(\enci{2}(\pi^{(2)})))$    
   % \State $(\ci{1}, \ci{2}) = (\enci{1}(\si{1}), \enci{2}(\si{2}))$
%        \State $(c_{\rm helper}, c_{\rm leader})=(\enc_{\rm helper}(s_{\rm helper}), \enc_{\rm leader}(s_{\rm leader}))$
        \Else
%            \State $(c_{\rm helper}, c_{\rm leader})=(\rerandomize_{\rm helper}(c_{\rm helper}), \rerandomize_{\rm leader}(c_{\rm leader}))$
    \State $(\ci{1}, \ci{2}) = (\rerandomizei{1}(\ci{1}), \rerandomizei{2}(\ci{2}))$   \label{step:rerandomize} 
    \State $(\pri{1}, \pri{2}) = (\rerandomizei{1}(\pri{1}), \rerandomizei{2}(\pri{2}))$
    \EndIf
    \EndFor
    \vspace{0.1in}

    \State \underline{\textbf{Send to Server}}
    \State $r={\rm Ber}(2/(e^{\epsilon_0}+1)$
    \If{$r=0$}
        \State $r'={\rm Ber}(1/2)$
        \If{$r'=1$}
    \State $(\si{1},\si{2})=\secretshare(0)$
  \State $(\pi^{(1)}, \pi^{(2)}) = \validityproof(\si{1},\si{2})$
    \State $(\ci{1}, \ci{2}) = (\rerandomizei{1}^t(\enci{1}(\si{1})), \rerandomizei{2}^t(\enci{2}(\si{2})))$
    \State $(\pri{1},\pri{2}) = (\rerandomizei{1}^t(\enci{1}(\pi^{(1)})),  \rerandomizei{2}^t(\enci{2}(\pi^{(2)})))$    
    % \State $(\ci{1}, \ci{2}) = (\enci{1}(\si{1}), \enci{2}(\si{2}))$
    % \State $(\pri{1},\pri{2}) = (\enci{1}(\pi^{(1)}),  \enci{2}(\pi^{(2)}))$    
%    \State $(\ci{1}, \ci{2}) = (\enci{1}(\si{1}), \enci{2}(\si{2}))$
%            \State $(s_{\rm helper}, s_{\rm leader})=\secretshare(0)$
%    \State $(c_{\rm helper}, c_{\rm leader})=(\enc_{\rm helper}(s^i_{\rm helper}), \enc_{\rm leader}(s^i_{\rm leader}))$
        \Else
    \State $(\si{1},\si{2})=\secretshare(1)$
      \State $(\pi^{(1)}, \pi^{(2)}) = \validityproof(\si{1},\si{2})$
    \State $(\ci{1}, \ci{2}) = (\rerandomizei{1}^{T}(\enci{1}(\si{1})), \rerandomizei{2}^T(\enci{2}(\si{2})))$
    \State $(\pri{1},\pri{2}) = (\rerandomizei{1}^{T}(\enci{1}(\pi^{(1)})),  \rerandomizei{2}^T(\enci{2}(\pi^{(2)})))$    
    % \State $(\ci{1}, \ci{2}) = (\enci{1}(\si{1}), \enci{2}(\si{2}))$
    % \State $(\pri{1},\pri{2}) = (\enci{1}(\pi^{(1)}),  \enci{2}(\pi^{(2)}))$    
%    \State $(\ci{1}, \ci{2}) = (\enci{1}(\si{1}), \enci{2}(\si{2}))$
%            \State $(s_{\rm helper}, s_{\rm leader})=\secretshare(1)$
%    \State $(c_{\rm helper}, c_{\rm leader})=(\enc_{\rm helper}(s^i_{\rm helper}), \enc_{\rm leader}(s^i_{\rm leader}))$
        \EndIf
      \EndIf
    \State $(\ci{1}, \ci{2}) = (\rerandomizei{1}(\ci{1}), \rerandomizei{2}(\ci{2}))$
    \State $(\pri{1}, \pri{2}) = (\rerandomizei{1}(\pri{1}), \rerandomizei{2}(\pri{2}))$
%        \State $(\pri{1},\pri{2}) = (\enci{1}(\pi^{(1)}),  \enci{2}(\pi^{(2)}))$    
%         \State $(c_{\rm helper}, c_{\rm leader})=(\rerandomize_{\rm helper}(c_{\rm helper}), \rerandomize_{\rm leader}(c_{\rm leader}))$    
  
    \State \textbf{Return} $(\ci{1}, \pri{1}, \ci{2}, \pri{2})$%$c_{\rm helper}, c_{\rm leader}$
    \end{algorithmic}
\end{algorithm}
\end{figure}
\algrenewcommand\algorithmicindent{2.0em}%

